Feature Distribution Shift Mitigation with Contrastive Pretraining for Intrusion Detection

In recent years, there has been a growing interest in using Machine Learning (ML), especially Deep Learning (DL) to solve Network Intrusion Detection (NID) problems. However, the feature distribution shift problem remains a difficulty, because the change in features' distributions over time negatively impacts the model's performance. As one promising solution, model pretraining has emerged as a novel training paradigm, which brings robustness against feature distribution shift and has proven to be successful in Computer Vision (CV) and Natural Language Processing (NLP). To verify whether this paradigm is beneficial for NID problem, we propose SwapCon, a ML model in the context of NID, which compresses shift-invariant feature information during the pretraining stage and refines during the finetuning stage. We exemplify the evidence of feature distribution shift using the Kyoto2006+ dataset. We demonstrate how pretraining a model with the proper size can increase robustness against feature distribution shifts by over 8%. Moreover, we show how an adequate numerical embedding strategy also enhances the performance of pretrained models. Further experiments show that the proposed SwapCon model also outperforms eXtreme Gradient Boosting (XGBoost) and K-Nearest Neighbor (KNN) based models by a large margin.

==> sections/04_tabpretrain.tex <==

\label{sec:tabpretrain}

Unlike images and free text, tabular data is highly structured and locally discontinuous, which means that we can change the order of columns or rows of a table and still read the information. But if we change the arrangement of pixels of an image or the order of words in a sentence, we can barely understand the data. This characteristic leads to different pre-training strategies for tabular data. 

 Since each piece of sample in a table is a row containing a series of features, one intuition suggested by \cite{tabpretrain} is to serialize a row into a sentence and then perform language model pre-training such as MLM. In \cite{turl}, Deng et al. decomposed the tabular pre-training into 3 steps: 
\begin{enumerate}
\item An encoding step to convert each row of feature values together with table meta-information into a sequence of tokens.
\item N stacked Transformer \cite{transformer} layers with structure-aware attention to capture the textual and structural information.
\item A projection layer to get the final representation for the learning objective function.
 \end{enumerate}
Likewise, TABBIE \cite{tabbie} chooses to linearize rows and columns separately and combine those two to get the final representation. There are many other works that follow this idea. \cite{transtab, tabert}

It is also possible to perform contrastive learning on tabular data. Somepalli et al. \cite{saint} proposed a pre-training framework that first applies augmentation operations on rows and trains a Transformer-based encoder using a contrastive objective function. Positive pairs are generated by mixing up several rows in a batch and the NCE loss function is used to minimize the 
